Stability of Influence Maximization

The present article serves as an erratum to our paper of the same title, which was presented and published in the KDD 2014 conference. In that article, we claimed falsely that the objective function defined in Section 1.4 is non-monotone submodular. We are deeply indebted to Debmalya Mandal, Jean Pouget-Abadie and Yaron Singer for bringing to our attention a counter-example to that claim. Subsequent to becoming aware of the counter-example, we have shown that the objective function is in fact NP-hard to approximate to within a factor of $O(n^{1-\epsilon})$ for any $\epsilon > 0$. In an attempt to fix the record, the present article combines the problem motivation, models, and experimental results sections from the original incorrect article with the new hardness result. We would like readers to only cite and use this version (which will remain an unpublished note) instead of the incorrect conference version.

==> IDM.tex <==
\section{Influence Difference Maximization Problem}
\label{sec:IDM}
It is impossible to directly evaluate (\ref{Equ:Inst1_4}) since the true influence strength parameters $\InfStrSU{\True}$ and thus $\OptSD{\True}$. Instead, we bound the term by
\begin{eqnarray}
\IMFuncD{\Max}{\OptSD{\True}} - \IMFuncD{\Obv}{\OptSD{\True}} & \leq & \arg\max_{\SeedS}[\IMFuncD{\Max}{\SeedS} - \IMFuncD{\Obv}{\SeedS}] \nonumber\\
& = & \alpha_2\cdot\IMFuncD{\Obv}{\AlgSD{\Obv}}\nonumber
\end{eqnarray}
In this section, we compute $\arg\max_{\SeedS}[\IMFuncD{\Max}{\SeedS} - \IMFuncD{\Obv}{\SeedS}]$ by solving a newly defined \emph{Influence Difference Maximization (IDM) Problem}. We prove that the objective function of IDM problem is submodular and then a random greedy algorithm is used to solve the problem efficiently and thus completing the upper bound for instability.

\subsection{Problem definition}
Informally, the IDM problem is to select a set of $k$ seeds, such that the difference in influence coverage under two sets of influence strength parameters is maximized.

More precisely, let $G=(V,E)$ be a social network and $\InfStrSU{\Pos}$ and $\InfStrSU{\Neg}$ be two sets of influence strength parameters. We require that for each parameter $\InfStrOD{i}$, we have $\InfStrOUD{\Pos}{i} \geq \InfStrOUD{\Neg}{i}$. For example, it requires $\ActProbUD{\Pos}{e}\geq \ActProbUD{\Neg}{e}, \forall e\in E$ under IC model and $\EdgeWUD{\Pos}{e}\geq \EdgeWUD{\Neg}{e}, \forall e\in E$ under LT model. The objection function $\IDMFuncD{\InfStrSU{\Pos},\InfStrSU{\Neg}}{\SeedS}$ is defined as
$$
\IDMFuncD{\InfStrSU{\Pos},\InfStrSU{\Neg}}{\SeedS} = \IMFuncD{\InfStrSU{\Pos}}{\SeedS} - \IMFuncD{\InfStrSU{\Neg}}{\SeedS},
$$
where $\IMFuncD{\InfStrSU{\Pos}}{\SeedS}$ and $\IMFuncD{\InfStrSU{\Neg}}{\SeedS}$ are objective functions for {\InfMax} under influence strength $\InfStrSU{\Pos}$ and $\InfStrSU{\Neg}$.
Then, the IDM problem is formulated as the following optimization problem:
$$
\begin{array}{cc}
  \text{Maximize} & \IDMFuncD{\InfStrSU{\Pos},\InfStrSU{\Neg}}{\SeedS}\\
  \text{Subject to} & |\SeedS|=k. \\
\end{array}
$$
When the context is clear, we drop $\InfStrSU{\Pos},\InfStrSU{\Neg}$ in the objective function to make it uncluttered as $\IDMFunc{\cdot}$.

The IDM problem differs from {\InfMax} problem in that: (1) The objective function of IDM problem is not monotone. Since we have $\IDMFunc{\emptyset}=\IDMFunc{V}=0$, but not necessary for any set between the two extremes; (2) The cardinality constraint for {\InfMax} problem is $|S|\leq k$, however, for IDM problem, it is a equality constraint $|S|=k$.

\subsection{Submodularity of $\IDMFuncD{\InfStrSU{\Pos},\InfStrSU{\Neg}}{\cdot}$}
The submodularity of set function $\delta(S)$ provides a good way
	to obtain an apporiximation algorithm for the IDM problem.
We say that a set function $f(S)$ with domain $2^V$ is {\em submodular} if
	for all $S\subseteq T \subseteq V$, and $x\not\in T$,
	we have $f(S\cup \{x\})-f(S) \ge f(T\cup \{x\})-f(T)$.
Intuitively, submodularity of $f$ means $f$ has the diminishing marginal
	return property.

 We now show that $\IDMFunc{\SeedS}$ is submodular by following the general methodology as in~\cite{InfluenceSpread} for the proof. However, our proof is more involved because we have multiple diffusion processes and careful coupling is in need to ensure submodularity under each possible random outcome.

\subsubsection{IC model}
We begin with the simple case, namely proving submodularity $\IDMFunc{\cdot}$ under IC model as a warm up and then proceed to the submodularity proof under LT model and the more complictaed GT model.

We establish the submodularity of $\delta(\cdot)$ by showing that
\begin{equation}\label{Equ:subIC}
\IDMFunc{S\cup\{v\}}-\IDMFunc{S}\geq \IDMFunc{T\cup\{v\}}-\IDMFunc{T}, \forall S\subseteq T\subseteq V.
\end{equation}
We use the same methodology in~\cite{InfluenceSpread} to prove the submodularity is true under each possible random outcome $\RC$. Different from the proof for {\InfMax}, we now have eight diffusion processes going on, namely
$$
\DP{A}{\InfStrSU{\Neg}}{S}, \DP{A}{\InfStrSU{\Neg}}{S\cup\Set{v}}, \DP{A}{\InfStrSU{\Neg}}{T}, \DP{A}{\InfStrSU{\Neg}}{T\cup\Set{v}}
$$
$$
\DP{A}{\InfStrSU{\Pos}}{S}, \DP{A}{\InfStrSU{\Pos}}{S\cup\Set{v}}, \DP{A}{\InfStrSU{\Pos}}{T}, \DP{A}{\InfStrSU{\Pos}}{T\cup\Set{v}}.
$$ We need to couple the random choices for all the eight processes. For the IC model, we take a naive coupling method by setting them all to the same random choice $X$. Instead of using the result of bias coin flipping for each edge as random choice~\cite{InfluenceSpread}, we draw a random number $r_e$ uniformly distribution in $[0,1]$ for each edge $e$. The corresponding edge $e$ is live if $r_e$ is greater or equal than the activation probability of the edge provided by the influence strength parameter $w_e$. Otherwise, the edge is blocked. For each process, we only keep the live edges and denote the resulted graph as \emph{live-edge} graph following~\cite{InfluenceSpread}. By this coupling method, the first four processes lead to the same live-edge graph $\GUD{\Pos}{\RC}=(V,E_{\RC}^\Pos)$ and the other four processes leads to the same live-edge graph $\GUD{\Neg}{\RC}=(V,E_{\RC}^\Neg)$. It is obvious that $E_{\RC}^-\subseteq E_{\RC}^+$.

Let $\RSFuncUD{\Pos}{\RC}{\SeedS}$ be the set of reachable nodes from seed set $S$ under graph $\GUD{\Pos}{\RC}$ and similarly $\RSFuncUD{\Neg}{\RC}{\SeedS}$. By results in~\cite{InfluenceSpread}, $\RSFuncUD{\Pos}{\RC}{\SeedS}$ equals the set of activated nodes by seed set $\SeedS$ and influence strength $\InfStrSU{\Pos}$ under random choices $\RC$ and similarly for $\RSFuncUD{\Neg}{\RC}{\SeedS}$. We also define $\DSFuncD{\RC}{\SeedS}=\RSFuncUD{\Pos}{\RC}{\SeedS}\backslash\RSFuncUD{\Neg}{\RC}{\SeedS}$, which is the set of nodes that are activated under influence strength $\InfStrSU{\Pos}$ but not under $\InfStrSU{\Neg}$. For clear presentation, we will drop $\RC$ when there is no ambiguity.

We will prove (\ref{Equ:subIC}) by showing that under any random choice $\RC$, $\forall S\subseteq T \subseteq V,$
\begin{equation}\label{Equ:subSetIC}
\DSFunc{T\cup\Set{v}}\backslash \DSFunc{T} \subseteq \DSFunc{S\cup\Set{v}}\backslash \DSFunc{S}.
\end{equation}

We first use next two lemmas to give the sufficient and necessary conditions for
$v\in \DSFunc{T}$ and $v\in \DSFunc{T\cup\Set{v}} \backslash \DSFunc{T}$ by the reachability  in live-edge graph $\GU{\Pos}$ and $\GU{\Neg}$.
\begin{lemma} \label{lem:SNCforD}
The sufficient and necessary condition for $u\in \DSFunc{T}$ is:
\vspace{-5 mm}
\begin{enumerate}
\setlength{\itemsep}{-1ex}
\item There exists a path from node set $T$ to $u$ in $\GU{\Pos}$.
\item There exists no path from node set $T$ to $u$ in $\GU{\Neg}$.
\end{enumerate}
\end{lemma}

\begin{lemma} \label{lem:SNCforDDet}
The sufficient and necessary
condition for $u\in \DSFunc{T\cup\Set{v}} \backslash \DSFunc{T}$ is:
\vspace{-5 mm}
\begin{enumerate}
\setlength{\itemsep}{-1ex}
\item There exists a path from node set $T\cup\{v\}$ to $u$ in $\GU{\Pos}$.
\item There exists no path from node set $T\cup\{v\}$ to $u$ in $\GU{\Neg}$.
\item There exists no path from node set $T$ to $u$ in $\GU{\Pos}$.
\end{enumerate}
\end{lemma}

With the above two lemmas, we prove (\ref{Equ:subSetIC}) with the following lemma.
\begin{lemma} \label{lem:SetSubIC}
$\forall S\subseteq T \subseteq V$ and $v\in V$, $\DSFunc{T\cup\Set{v}} \backslash \DSFunc{T} \subseteq \DSFunc{S\cup\Set{v}} \backslash \DSFunc{S}$.
\end{lemma}
\vspace{-5 mm}
\begin{proof}
For any $u\in \DSFunc{T\cup\Set{v}} \backslash \DSFunc{T}$ ,we prove $u\in \DSFunc{S\cup\Set{v}} \backslash \DSFunc{S}$ by showing all three conditions in Lemma~\ref{lem:SNCforDDet} are satisfied. The satisfaction of condition 2 and 3 are obvious, since we switch from $T$ to a smaller set $S$. By combining condition 1 and 3 for set $T$, we know there must exists a path from the node $v$ to $u$ in $\GU{\Pos}$, which suggests that there is also a path from $S\cup\{v\}$ to $u$ in $\GU{\Pos}$. This implies the satisfaction of condition 1 and thus completes the proof.
\end{proof}
\vspace{-5 mm}
\begin{theorem}
For an arbitrary instance of IDM problem under IC model, the objective function $\delta(\cdot)$ is submodular.
\end{theorem}
\vspace{-5 mm}
\begin{proof}
\begin{flalign*}
& \ \ \ \ \ [\IDMFunc{S\cup\{v\}}-\IDMFunc{S}] - [\IDMFunc{T\cup\{v\}}-\IDMFunc{T}]\nonumber\\
& =  \sum_{\RC}\Prob{\RC}\cdot(|\DSFunc{S\cup\Set{v}} \backslash \DSFunc{S}| - |\DSFunc{T\cup\Set{v}} \backslash \DSFunc{T}|) \nonumber\\
& \geq 0\nonumber\\
\end{flalign*}
Since the non-negative linear combination of submodular functions are still submodular, thus we have proved the submodularity of the objective function.
\end{proof}
\subsubsection{LT model}
The proof of submodularity under LT model is similar to that under IC model in terms of coupling all the eight processes with the same random choice $\RC$. However, the way we use the random choices to derive the live-edge graphs is more involved.

Basically, we follow the same approach in~\cite{InfluenceSpread} to derive the live-edge graph. Namely, for each node $u$, we pick at most one of the incoming edge at random with probability $\EdgeWD{v,u}$ and select no edge with probability $1-\sum_v \EdgeWD{v,u}$. The selected edge is set to live while all other edges are blocked. In has been proved in~\cite{InfluenceSpread} that the reachable nodes under the live-edge graph are exactly the activated nodes under LT model.

For our purpose, we consider the following procedure for picking the live edges. For each node $v$, we have an interval $[0,1]$. Then, for every incoming edge $\langle u,v\rangle$, we place an interval with length $\EdgeWD{u,v}$ without overlapping into the $[0,1]$ interval. Then a random number $r_v$ is drawn uniformly at random from $[0,1]$, if $r_v$ lies in the interval associated with an edge $\langle u,v\rangle$, we let $\langle u,v\rangle$ to be live. Otherwise, we block all incoming edges for node $v$.

We first carry out the above procedure with influence strength parameters $\InfStrSU{\Pos}$. Then, for the processes with influence strength $\InfStrSU{\Neg}$, we align the starting point for each incoming edge. The procedure is illustrated with the example shown in Figure~\ref{Fig:LRCoupling}.
\begin{figure}[!h]
  \centering
  \includegraphics[width=0.5\textwidth]{./figures/LRCoupling.png}
  \caption{Example of coupling for submodulairy proof under LT model.}\label{Fig:LRCoupling}
\end{figure}
In this example, we consider drawing the live edge for node $v$, who has three incoming neighbours $x,y,z$, under both $\InfStrSU{\Pos}$ and $\InfStrSU{\Neg}$. We first place the interval for $\EdgeWUD{\Pos}{x,v}$, $\EdgeWUD{\Pos}{y,v}$ and $\EdgeWUD{\Pos}{z,v}$ without overlapping. Then we put the interval for $\EdgeWUD{\Neg}{x,v}$, $\EdgeWUD{\Neg}{y,v}$ and $\EdgeWUD{\Neg}{z,v}$ on the upper segment by left alignment. Finally, an number $r_e$ is drawn uniformly at random to decide the live-edge for both $\GU{\Pos}$ and $\GU{\Neg}$. From the construction, it is obvious that we also have $E^{\Neg}\subseteq E^{\Pos}$ as that under IC model. The rest part of the submodularity proof is exactly the same as that for live-edge graph under IC model.

\subsubsection{GT model}
The proof of submodularity under GT model is more complicated than that under IC and LT model, since we no longer have the live-graph in which we can characterize the activated nodes by reachability. Moreover, the simple coupling method by using same random choice for all diffusion processes fails.

However, we still use coupling method and prove the submodularity under each random choices, however the complex coupling method proposed by Moseel and Roch in~\cite{Elchanan:Sebastien:submodularity}.

We first couple the four processes
\begin{eqnarray}
& &\bm{A}^{\Pos}=\DP{A}{\InfStrSU{\Pos}}{S}\nonumber\\
& &\bm{B}^{\Pos}=\DP{B}{\InfStrSU{\Pos}}{S\cup\Set{v}}\nonumber\\
& &\bm{C}^{\Pos}=\DP{C}{\InfStrSU{\Pos}}{T}\nonumber\\
& &\bm{D}^{\Pos}=\DP{D}{\InfStrSU{\Pos}}{T\cup\Set{v}}\nonumber
\end{eqnarray}
by setting $A=S\cup\{v\}, B=T, C=S,D=T\cup\{v\}$ as the corresponding processes defined in~\cite{Elchanan:Sebastien:submodularity}. For the other four processes with $\InfStrSU{\Neg}$, namely
\begin{eqnarray}
& &\bm{A}^{\Neg}=\DP{A}{\InfStrSU{\Neg}}{S}\nonumber\\
& &\bm{B}^{\Neg}=\DP{B}{\InfStrSU{\Neg}}{S\cup\Set{v}}\nonumber\\
& &\bm{C}^{\Neg}=\DP{C}{\InfStrSU{\Neg}}{T}\nonumber\\
& &\bm{D}^{\Neg}=\DP{D}{\InfStrSU{\Neg}}{T\cup\Set{v}},\nonumber
\end{eqnarray}
we couple them with exactly the same random choices as we do for the four processes with $\InfStrSU{\Pos}$.

Then, similarly we have the following lemma. Here we abuse the notation by using $\RSUD{DP}{\RC}$ to denote the set of activated nodes by the end of process $DP$ under random choice $\RC$. Also, for simplicity, we omit the subscript $\RC$.
\begin{lemma} \label{lem:SNCforDDetGT}
The sufficient and necessary
condition for $u\in \DSFunc{T\cup\Set{v}} \backslash \DSFunc{T} \subseteq \DSFunc{S\cup\Set{v}} \backslash \DSFunc{S}$ is:
\vspace{-5 mm}
\begin{enumerate}
\setlength{\itemsep}{-0.5ex}
\item $u \in \RSU{\bm{D}^{\Pos}}$
\item $u \not\in \RSU{\bm{D}^{\Neg}}$
\item $u \not\in \RSU{\bm{C}^{\Pos}}$
\end{enumerate}
\end{lemma}
\begin{lemma} \label{lem:SetSubGT}
$\forall S\subseteq T \subseteq V$ and $v\in V$, $\DSFunc{T\cup\Set{v}} \backslash \DSFunc{T} \subseteq \DSFunc{S\cup\Set{v}} \backslash \DSFunc{S}$.
\end{lemma}
\vspace{-5 mm}
\begin{proof}
For any $u\in D(T\cup\{v\})\backslash D(T)$ ,we prove $u\in \DSFunc{T\cup\Set{v}} \backslash \DSFunc{T}$ bu showing all three conditions in Lemma~\ref{lem:SNCforDDetGT} are satisfied, namely (1)$u \in \RSU{\bm{B}^{\Pos}}$; (2)$u \not\in \RSU{\bm{B}^{\Neg}}$; (3)$u \not\in \RSU{\bm{A}^{\Pos}}$. The satisfaction of condition (2) and (3) are obvious, since we switch the seed set from $T$ to a smaller set $S$. By the coupling method in~\cite{Elchanan:Sebastien:submodularity}, we know
$$
\RSU{\bm{D}^{\Pos}}\backslash \RSU{\bm{C}^{\Pos}} \subseteq
\RSU{\bm{B}^{\Pos}}\backslash \RSU{\bm{A}^{\Pos}}.
$$
Since $u\in \RSU{\bm{D}^{\Pos}}\backslash \RSU{\bm{C}^{\Pos}}$ and $u\not\in \RSU{\bm{A}^{\Pos}}$, we conclude that $\RSU{\bm{B}^{\Pos}}$, which completes the proof.
\end{proof}

\subsection{Random greedy algorithm}
In this section, we utilize the submodularity to design an efficient algorithm to solve the IDM problem. Due to the non-monotonicity and the exact cardinality constraint, the simple greedy algorithm is no longer capable to provide any approximation guarantee~\cite{Buchbinder:Feldman:Naor:Schwartz}.

Instead, we resort to the \emph{Random Greedy} algorithm proposed in~\cite{Buchbinder:Feldman:Naor:Schwartz}. The pseudo-code of the algorithm is shown in Algorithm~\ref{Alg:RandomGreedy}.

\begin{algorithm}[h]
\caption{Random Greedy}\label{Alg:RandomGreedy}
\begin{algorithmic}[1]
\STATE Initialize: $S_0\leftarrow\emptyset$
\FOR{i=1 to k}
\STATE Let $M_i\subseteq V\backslash S_{i-1}$ be the subset of size k maximizing $\sum_{u\in M_i}\IDMFunc{S_{i-1}\cup\{u\}}-\IDMFunc{S_{i-1}}$.
\STATE Draw $u_i$ uniformly ar random from $M_i$.
\STATE $S_i\leftarrow S_{i-1}\cup\{u_i\}$
\ENDFOR
\STATE Return $S_k$
\end{algorithmic}
\end{algorithm}
The structure of the algorithm is quite similar to the greedy algorithm used for {\InfMax}. Instead of adding the element with maximal marginal gain, we first pickup the $k$ nodes with maximum marginal gains as set $M_i$. Then, a node is selected uniformly at random from the set and is added to the result set. It has been proved that in expectation the above algorithm leads to a $\frac{1-k/e|V|}{e}-\varepsilon$ approximation guarantee. We choose this particular algorithm instead of other ones with even tighter bound~\cite{Buchbinder:Feldman:Naor:Schwartz} mainly due to its simplicity and efficiency. The running time of the algorithm is $O(kC|V|)$, where $C$ is the time used in estimating $\IDMFunc{S\cup\{u\}}-\IDMFunc{S}$ by Monte-Carlo simulation. We have $C=O(T|V|)$, $T$ is the times we run Monte-Carlo simulations. The overall running time becomes $O(kT|V|^2)$. In order to accelerate the algorithm, we optimize the algorithm with the CELF method proposed by Jure et al. in~\cite{LKGFVG}.

